The splitting in potential Crank-Nicolson scheme with discrete transparent boundary conditions for the Schr\"odinger equation on a semi-infinite strip

We consider an initial-boundary value problem for a generalized 2D time-dependent Schr�odinger equation (with variable coefficients) on a semi-infinite strip. For the Crank-Nicolson-type finite-difference scheme with approximate or discrete transparent boundary conditions (TBCs), the Strang-type splitting with respect to the potential is applied. For the resulting method, the unconditional uniform in time $L^2$-stability is proved. Due to the splitting, an effective direct algorithm using FFT is developed now to implement the method with the discrete TBC for general potential. Numerical results on the tunnel effect for rectangular barriers are included together with the detailed practical error analysis confirming nice properties of the method.

==> table.B.1500.error.J_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$J$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{C}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{L^2}$}&\multicolumn {2}{c}{$T\,\,{\rm sec.}$}&\multicolumn {2}{c}{$R_{\rm time}$}\\\midrule %
$300$&$$&$0$&$.22$&--&&$0$&$.12$&--&&$1\,144$&$$&--&\\%
$600$&$$&$5$&$.62\cdot 10^{-2}$&$3$&$.99$&$3$&$.10\cdot 10^{-2}$&$3$&$.94$&$1\,526$&$$&$1$&$.33$\\%
$1\,200$&$$&$1$&$.42\cdot 10^{-2}$&$3$&$.95$&$7$&$.91\cdot 10^{-3}$&$3$&$.92$&$2\,236$&$$&$1$&$.47$\\%
$2\,400$&$$&$3$&$.77\cdot 10^{-3}$&$3$&$.77$&$2$&$.16\cdot 10^{-3}$&$3$&$.66$&$3\,644$&$$&$1$&$.63$\\%
$4\,800$&$$&$1$&$.20\cdot 10^{-3}$&$3$&$.15$&$7$&$.65\cdot 10^{-4}$&$2$&$.83$&$6\,605$&$$&$1$&$.81$\\\bottomrule %
\end {tabular}%


==> table.B.1500.error.K_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$K$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{C}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{L^2}$}&\multicolumn {2}{c}{$T\,\,{\rm sec.}$}&\multicolumn {2}{c}{$R_{\rm time}$}\\\midrule %
$16$&$$&$0$&$.15$&--&&$6$&$.62\cdot 10^{-2}$&--&&$466$&$$&--&\\%
$32$&$$&$3$&$.43\cdot 10^{-2}$&$4$&$.36$&$2$&$.34\cdot 10^{-2}$&$2$&$.84$&$996$&$$&$2$&$.13$\\%
$64$&$$&$8$&$.65\cdot 10^{-3}$&$3$&$.96$&$6$&$.58\cdot 10^{-3}$&$3$&$.55$&$1\,898$&$$&$1$&$.91$\\%
$128$&$$&$2$&$.29\cdot 10^{-3}$&$3$&$.79$&$1$&$.81\cdot 10^{-3}$&$3$&$.63$&$3\,523$&$$&$1$&$.86$\\%
$256$&$$&$1$&$.20\cdot 10^{-3}$&$1$&$.91$&$7$&$.65\cdot 10^{-4}$&$2$&$.37$&$6\,605$&$$&$1$&$.87$\\\bottomrule %
\end {tabular}%


==> table.B.1500.error.M_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$M$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{C}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$R_{L^2}$}&\multicolumn {2}{c}{$T\,\,{\rm sec.}$}&\multicolumn {2}{c}{$R_{\rm time}$}\\\midrule %
$150$&$$&$0$&$.17$&--&&$9$&$.10\cdot 10^{-2}$&--&&$368$&$$&--&\\%
$300$&$$&$4$&$.39\cdot 10^{-2}$&$3$&$.91$&$2$&$.37\cdot 10^{-2}$&$3$&$.84$&$774$&$$&$2$&$.1$\\%
$600$&$$&$1$&$.12\cdot 10^{-2}$&$3$&$.9$&$6$&$.20\cdot 10^{-3}$&$3$&$.83$&$1\,567$&$$&$2$&$.02$\\%
$1\,200$&$$&$3$&$.16\cdot 10^{-3}$&$3$&$.56$&$1$&$.83\cdot 10^{-3}$&$3$&$.39$&$3\,157$&$$&$2$&$.01$\\%
$2\,400$&$$&$1$&$.20\cdot 10^{-3}$&$2$&$.64$&$7$&$.65\cdot 10^{-4}$&$2$&$.39$&$6\,605$&$$&$2$&$.09$\\\bottomrule %
\end {tabular}%


==> table.B.1500.ssp.comparison_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$J$}&\multicolumn {2}{c}{$K$}&\multicolumn {2}{c}{$M$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$P_{C}$}&\multicolumn {2}{c}{$P_{L^2}$}\\\midrule %
$1\,200$&$$&$64$&$$&$600$&$$&$2$&$.54\cdot 10^{-2}$&$1$&$.60\cdot 10^{-2}$&$-5$&$.65$&$-3$&$.08$\\%
$1\,200$&$$&$128$&$$&$600$&$$&$2$&$.42\cdot 10^{-2}$&$1$&$.37\cdot 10^{-2}$&$-6$&$.6$&$-3$&$.78$\\%
$1\,200$&$$&$64$&$$&$1\,200$&$$&$1$&$.83\cdot 10^{-2}$&$1$&$.21\cdot 10^{-2}$&$0$&$.36$&$-0$&$.91$\\%
$1\,200$&$$&$128$&$$&$1\,200$&$$&$1$&$.63\cdot 10^{-2}$&$9$&$.40\cdot 10^{-3}$&$-2$&$.49$&$-1$&$.33$\\%
$2\,400$&$$&$64$&$$&$600$&$$&$1$&$.64\cdot 10^{-2}$&$1$&$.09\cdot 10^{-2}$&$-5$&$.48$&$-3$&$.99$\\%
$2\,400$&$$&$128$&$$&$600$&$$&$1$&$.38\cdot 10^{-2}$&$8$&$.05\cdot 10^{-3}$&$-11$&$.39$&$-6$&$.27$\\%
$2\,400$&$$&$64$&$$&$1\,200$&$$&$1$&$.03\cdot 10^{-2}$&$7$&$.73\cdot 10^{-3}$&$1$&$.01$&$-0$&$.96$\\%
$2\,400$&$$&$128$&$$&$1\,200$&$$&$6$&$.00\cdot 10^{-3}$&$3$&$.82\cdot 10^{-3}$&$-6$&$.3$&$-3$&$.02$\\\bottomrule %
\end {tabular}%


==> table.B.4000.error_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$J$}&\multicolumn {2}{c}{$K$}&\multicolumn {2}{c}{$M$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$E_{C,\,{\rm rel}}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm rel}}$}\\\midrule %
$2\,400$&$$&$64$&$$&$600$&$$&$8$&$.61\cdot 10^{-3}$&$5$&$.29\cdot 10^{-3}$&$2$&$.48\cdot 10^{-2}$&$2$&$.90\cdot 10^{-2}$\\%
$1\,200$&$$&$128$&$$&$600$&$$&$1$&$.38\cdot 10^{-2}$&$6$&$.37\cdot 10^{-3}$&$3$&$.56\cdot 10^{-2}$&$2$&$.82\cdot 10^{-2}$\\%
$1\,200$&$$&$64$&$$&$1\,200$&$$&$1$&$.22\cdot 10^{-2}$&$5$&$.30\cdot 10^{-3}$&$2$&$.82\cdot 10^{-2}$&$2$&$.33\cdot 10^{-2}$\\\bottomrule %
\end {tabular}%


==> table.C.1500.error_old.tex <==
\begin {tabular}{r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \multicolumn {2}{c}{$J$}&\multicolumn {2}{c}{$K$}&\multicolumn {2}{c}{$M$}&\multicolumn {2}{c}{$E_{C,\,{\rm abs}}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm abs}}$}&\multicolumn {2}{c}{$E_{C,\,{\rm rel}}$}&\multicolumn {2}{c}{$E_{L^2,\,{\rm rel}}$}\\\midrule %
$2\,400$&$$&$512$&$$&$600$&$$&$1$&$.06\cdot 10^{-2}$&$5$&$.26\cdot 10^{-3}$&$3$&$.16\cdot 10^{-2}$&$2$&$.32\cdot 10^{-2}$\\%
$1\,200$&$$&$1\,024$&$$&$600$&$$&$9$&$.64\cdot 10^{-3}$&$6$&$.70\cdot 10^{-3}$&$3$&$.92\cdot 10^{-2}$&$4$&$.38\cdot 10^{-2}$\\%
$1\,200$&$$&$512$&$$&$1\,200$&$$&$8$&$.22\cdot 10^{-3}$&$4$&$.67\cdot 10^{-3}$&$2$&$.66\cdot 10^{-2}$&$2$&$.06\cdot 10^{-2}$\\\bottomrule %
\end {tabular}%


==> table.tex <==
\pgfplotstableset{%
    empty cells with={--}, % replace empty cells with '--'
    every head row/.style={%
        before row=\toprule, after row=\midrule
    },
%    every even row/.style={%
%        before row={\rowcolor[gray]{0.9}}
%    },
    every last row/.style={%
        after row=\bottomrule
    },
    col sep=comma,
    1000 sep={\,},
    dec sep align,
    sci zerofill,
}
\pgfplotstableread{data/table.B.1500.error.J.csv}\dataJ
\pgfplotstableread{data/table.B.1500.error.K.csv}\dataK
\pgfplotstableread{data/table.B.1500.error.M.csv}\dataM
\pgfplotstableread{data/table.B.1500.ssp.comparison.csv}\dataComp
\pgfplotstableread{data/table.B.4000.error.csv}\dataF
\pgfplotstableread{data/table.C.1500.error.csv}\dataC
%
\par\pgfplotstabletypeset[%
%    row predicate/.code={%
%        \pgfplotstablegetelem{#1}{[index]1}\of{\data}
%        \ifnum\pgfplotsretval=1200
%            \pgfplotstablegetelem{#1}{[index]2}\of{\data}
%            \ifnum\pgfplotsretval=128
%                \relax
%            \else
%                \pgfplotstableuserowfalse
%            \fi
%        \else
%            \pgfplotstableuserowfalse
%        \fi
%    },
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={7}},
    columns={[index]0,[index]3,rCa,[index]4,rLa,ct},%,[index]7
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_C$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh})}$
    columns/4/.style={column name=$E_{L^2}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh}}$
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh}),\,{\rm rel}}$
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh},\,{\rm rel}}$
%    columns/7/.style={column name=$T\,\,{\rm sec.}$, int trunc,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=table.B.1500.error.J.tex
]{\dataJ}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={7}},
    columns={[index]2,[index]3,rCa,[index]4,rLa,ct},%,[index]7
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
%    columns/7/.style={column name=$T\,\,{\rm sec.}$, int trunc,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=table.B.1500.error.K.tex
]{\dataK}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={7}},
    columns={[index]1,[index]3,rCa,[index]4,rLa,ct},%,[index]7
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
%    columns/7/.style={column name=$T\,\,{\rm sec.}$, int trunc,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=table.B.1500.error.M.tex
]{\dataM}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    columns={[index]0,[index]2,[index]1,[index]3,[index]4,[index]5,[index]6},
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$P_{C}$,},
    columns/6/.style={column name=$P_{L^2}$,},
    outfile=table.B.1500.ssp.comparison.tex
]{\dataComp}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    columns={[index]0,[index]2,[index]1,[index]3,[index]4,[index]5,[index]6},
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    outfile=table.B.4000.error.tex
]{\dataF}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    columns={[index]0,[index]2,[index]1,[index]3,[index]4,[index]5,[index]6},
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    outfile=table.C.1500.error.tex
]{\dataC} 
